Interferences in match kernels

We consider the design of an image representation that embeds and aggregates a set of local descriptors into a single vector. Popular representations of this kind include the bag-of-visual-words, the Fisher vector and the VLAD. When two such image representations are compared with the dot-product, the image-to-image similarity can be interpreted as a match kernel. In match kernels, one has to deal with interference, i.e. with the fact that even if two descriptors are unrelated, their matching score may contribute to the overall similarity. We formalise this problem and propose two related solutions, both aimed at equalising the individual contributions of the local descriptors in the final representation. These methods modify the aggregation stage by including a set of per-descriptor weights. They differ by the objective function that is optimised to compute those weights. The first is a "democratisation" strategy that aims at equalising the relative importance of each descriptor in the set comparison metric. The second one involves equalising the match of a single descriptor to the aggregated vector. These concurrent methods give a substantial performance boost over the state of the art in image search with short or mid-size vectors, as demonstrated by our experiments on standard public image retrieval benchmarks.

==> bow.tex <==
% !TEX root = paper.tex
\section{The bag-of-words case}
\label{sec:bow}

In this section, we discuss the particular case of our methods when applied to the bag-of-word representation with cosine similarity. We do not consider inverse-document-frequency terms. 

\subsection{Democratic aggregation: square-root normalisation}


\subsection{GMP and max-pooling}


%We can also study the BOV in the regularised case.
%Again, assuming hard assignment, $\p(x_i)$ is binary with a single entry corresponding
%to the codeword index. 
%Therefore $\Phi \1$ corresponds to the (unnormalised) BOV histogram
%and $\Phi \Phi^T$ is a diagonal matrix with the BOV histogram on the diagonal.
%%Then $\p_i \p_i^T$ is a matrix with zeros everywhere and a single 1 on the diagonal.
%%Therefore, we have $\bar{\p}$ the standard BOV vector obtained by average pooling and $C$ is the diagonal
%%matrix with $\bar{\p}$ on the diagonal: $C = \mbox{diag}(\bar{\p})$.
%In such a case, equation (\ref{eqn:primalsolreg}) rewrites as
%%
%\begin{equation}
%\p^*_{\lbd} = \frac{\Phi \1}{\Phi \1 + \lbd},
%\end{equation}
%%
%where the previous division should be understood as a term-by-term operation.
%With $\lbd$ infinitely small, we again recover the standard max-pooling mechanism.

%We now study the case of a non-orthonormal basis.
%Since this is much more difficult, we restrict ourselves to the case where we have two entries in the codebook: $q_1$ and $q_2$.

